Comparing School Choice and College Admission Mechanisms By Their Immunity to Strategic Admissions

Recently dozens of school districts and college admissions systems around the world have reformed their admission rules. As a main motivation for these reforms the policymakers cited strategic flaws of the rules: students had strong incentives to game the system, which caused dramatic consequences for non-strategic students. However, almost none of the new rules were strategy-proof. We explain this puzzle. We show that after the reforms the rules became more immune to strategic admissions: each student received a smaller set of schools that he can get in using a strategy, weakening incentives to manipulate. Simultaneously, the admission to each school became strategy-proof to a larger set of students, making the schools more available for non-strategic students. We also show that the existing explanation of the puzzle due to Pathak and S\"onmez (2013) is incomplete.

==> list.tex <==
+ Lars Ehlers
+ William Thomson
+ Herve Moulin (?)
+ Anna Bogomolnaia
+ Fedor
+ Kostya
+ Fuhito Kojima
+ Alvin Roth
+ Marek Pycia
+ Onur Kesten
+ Yan Chen
Umut Dur
+ Peter Troyan 
+ Thayer Morrill
Utku Unver
Tommy Anderson
Peter Biro
Peter Manlove (?)
Inacio Bo
Battal Dogan
Bettina Klaus
Haluk Ergin
Attila Abdulkadiroglu
Olivier 
Julien
+ Rustam


Please find our new paper attached. In the paper we explain the recent reforms in school choice systems around the world using a new concept called strategic accessibility. We also provide a counterexample showing that the state-of-the-art explanation using manipulability notion (Pathak and Sonmez, AER 2013) is incorrect for reforms in England and Wales.

We are wondering where to send it. We first submitted the counterexample to AER as a comment, but were not granted a publication. Now we developed our notion (which seems to us more intuitive, though we might be biased) to fill the gap. We would be very thankful for your feedback and suggestions.
